A standard theorem on adjunctions in two variables

We record an explicit proof of the theorem that lifts a two-variable adjunction to the arrow categories of its domains.

==> dis-preambolo.tex <==
\usepackage[all,cmtip]{xy}

\usepackage{xparse,amsmath,xcolor,amssymb,amsfonts}

\input{symbols}
